Learning Disentangled Representation in Object-Centric Models for Visual Dynamics Prediction via Transformers

Recent work has shown that object-centric representations can greatly help improve the accuracy of learning dynamics while also bringing interpretability. In this work, we take this idea one step further, ask the following question: "can learning disentangled representation further improve the accuracy of visual dynamics prediction in object-centric models?" While there has been some attempt to learn such disentangled representations for the case of static images \citep{nsb}, to the best of our knowledge, ours is the first work which tries to do this in a general setting for video, without making any specific assumptions about the kind of attributes that an object might have. The key building block of our architecture is the notion of a {\em block}, where several blocks together constitute an object. Each block is represented as a linear combination of a given number of learnable concept vectors, which is iteratively refined during the learning process. The blocks in our model are discovered in an unsupervised manner, by attending over object masks, in a style similar to discovery of slots \citep{slot_attention}, for learning a dense object-centric representation. We employ self-attention via transformers over the discovered blocks to predict the next state resulting in discovery of visual dynamics. We perform a series of experiments on several benchmark 2-D, and 3-D datasets demonstrating that our architecture (1) can discover semantically meaningful blocks (2) help improve accuracy of dynamics prediction compared to SOTA object-centric models (3) perform significantly better in OOD setting where the specific attribute combinations are not seen earlier during training. Our experiments highlight the importance discovery of disentangled representation for visual dynamics prediction.

==> checklist.tex <==

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly states the contribution. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
    %     \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
    %     \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
    %     \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    % \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
    %     \item The authors are encouraged to create a separate "Limitations" section in their paper.
    %     \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
    %     \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
    %     \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
    %     \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
    %     \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    %     \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    % \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}.
    \item[] Justification: \justificationTODO{}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include theoretical results. 
    %     \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
    %     \item All assumptions should be clearly stated or referenced in the statement of any theorems.
    %     \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
    %     \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
    %     \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    % \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{},% \answerNo{}, or \answerNA{}.
    \item[] Justification: We have provided all the hyper parameters and training, evaluation setup in paper
    %\item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    %     \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
    %     \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    %     \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    %     \begin{enumerate}
    %         \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
    %         \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
    %         \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
    %         \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    %     \end{enumerate}
    % \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} %, or \answerNA{}.
    \item[] Justification: Code, data and models will be released post acceptance. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that paper does not include experiments requiring code.
    %     \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
    %     \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
    %     \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
    %     \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
    %     \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    % \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} %, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have provided hyperparameters in the appendix. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
    %     \item The full details can be provided either with the code, in appendix, or as supplemental material.
    % \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:  \answerYes{}
    \item[] Guidelines: The results with uncertainity is added in the appendix. 
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    %     \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
    %     \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
    %     \item The assumptions made should be given (e.g., Normally distributed errors).
    %     \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
    %     \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
    %     \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
    %     \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    % \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} %, \answerNo{}, or \answerNA{}.
    \item[] Justification: Mentioned in the appendix 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
    %     \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
    %     \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    % \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer:\answerYes{} %, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the appendix
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that there is no societal impact of the work performed.
    %     \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
    %     \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
    %     \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
    %     \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
    %     \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    % \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer:  \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper poses no such risks.
    %     \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
    %     \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
    %     \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    % \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All the authors and people have been referred
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not use existing assets.
    %     \item The authors should cite the original paper that produced the code package or dataset.
    %     \item The authors should state which version of the asset is used and, if possible, include a URL.
    %     \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
    %     \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
    %     \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
    %     \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
    %     \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    % \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer:  \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
    %     \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    % \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer:\answerNA{}.
    % \item[] Justification: \justificationTODO{}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
    %     \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
    %     \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    % \end{itemize}

\end{enumerate}


==> intro_v0.tex <==
\section{Introduction}
\label{sec:intro}
Predicting visual dynamics is an important problem that finds applications in computer vision, model-based reinforcement learning, and visual question answering. Some of the classic work does this by having dense representation for the image and then passing through a CNN-based or now transformer-based architecture. More recent approaches have argued for the use of object-centric representations, presumably because they can better capture the natural semantics of how objects are represented in a scene and their interactions, for the task of dynamics prediction. This line of work can further be divided into two sets of categories: ones that work with dense object embeddings learned from the data~\cite{wu2023slotformer} and those that try to decompose each object representation in terms of its attributes~\cite{Neural-Systematic-Binder}. While in the former category, the latest models exploit the power of transformers to get the future dynamics, works in the second category have exploited autoencoder-based models, or GNN-based models, to learn disentangled representation for downstream learning of dynamics. Interestingly, some of the SOTA models~\cite{wu2023slotformer} do not use disentangled representation, leaving a possibility of further improvement in performance on this task while having a more interpretable representation.
%well as having better interpretability.
%via learning a disentangeled representation.

%Among the existing techniques which work with disentangled representation, they either make limiting assumptions about object attributes such as size, making them non-transferable~\cite{Stove}, make use of a hard-coded number of concepts independent of problem space~\cite{GSWM}, or segregate object factors into only two categories: those relevant for dynamics prediciton, and those which are not. There is some recent work by ~\cite{Neural-Systematic-Binder} on disocvering object concepts, but their work is limites to the setting of static images. Motivated by this research gap, we propose an approach for learning disentangled object representations, expressed as a linear combination of learnable concepts, for the task of visual dynamics prediction via transformers. Unlike earlier works, our approach is flexible to choose the number of concepts based on the problem space (as a hyperparameters), and our dynamics engine is based on transformers, exploiting some of the latest advances in the field for future sequence prediction.

%In other words, we combine the power of disentangled representations with the power of transorformers.


%Our approach is oblivious to the choice of object extractor.


%push the boundaries on two fronts: (1) Work with a more flexible disentangled representaition, which does \vscom{Does or does not?} apriori assume a fixed set of concepts, which is the same for every problem size. (2) Combine the learned representation with power of transformer based architectures, which have been shown to do very well on future prediction tasks, by allowing discovered latent factors (called {\em blocks} in our terminology) to attend on each other \vscom{The line reads too complicated, need to rewrite it}. We refer to our system as {\em DisFormer}.

%are limited to the stati
%And non of these exploit the power of transformers which have been shown to provide SOTA results for the task of unsupervised video prediction.
Even among the techniques that make use of a disentangled object representation, they are limited by their assumptions: (1) They either work with objects of the same size~\cite{kossen2019structured} (2) Or divide the attributes only into two sets: those relevant for dynamics, vs which are not~\cite{STEADY}. Both these assumptions are pretty restrictive. The closest to our work is ~\cite{lin2020improving}, which can learn disentangled representations, but it does it with a fixed number of concepts independent of the problem space. As observed in our experiments, this severely affects their performance, especially in the setting of transfer, for instance, where certain attribute combinations are never seen before. Motivated by these research gaps, we push the boundaries on two fronts: (1) Work with a more flexible disentangled representation, which can choose the number of concepts depending on the specific problem; (2) Combine the learned representation with the power of transformer-based architectures, which have been shown to do very well on future prediction tasks. We refer to our system as {\em DisFormer}.

%by allowing discovered latent factors (called {\em blocks} in our terminology) to attend on each other \vscom{The line reads too complicated, need to rewrite it}. 
%rather allowing the flexibility of introducing additional concepts.}
%\sout{comes to close to our work, by learning disentangled representations, but they do it with a fixed set of concepts independent of the problem space, rather allowing the flexibility of introducing additional concepts.} 
%\vscom{Don't we also have fixed combination of concept?}
%Accordingly, the level of distentangelement obtained by them is limited by this assumption, and 
%Further, they do not explicitly make use of learned representation in the dynamics prediction module, resulting in sub-optimal performance, especially when dealing with transfer settings, with object combinations never seen before. Inspired by this research gap, we push the boundaries on two fronts: (1) Work with a more flexible disentangled representaition, which does \vscom{Does or does not?} apriori assume a fixed set of concepts, which is the same for every problem size. (2) Combine the learned representation with power of transformer based architectures, which have been shown to do very well on future prediction tasks, by allowing discovered latent factors (called {\em blocks} in our terminology) to attend on each other \vscom{The line reads too complicated, need to rewrite it}. We refer to our system as {\em DisFormer}.

%On the other hand, we combine the power of transformers with learned disentangled representations which are a function of a small set of concepts, so that learned representation in terms of {\em object blocks} explicitly guides the working of transformer for future dynamics prediction.

%behave in real-world, resulting in better predictions~\cite{wu2023slotformer}
%In general, the task is unsupervised, i.e., no annotatinothat has received significant attention in the recent literature. It has a wide variety of applications including in video analysis and prediction, model based reinforcement learning, and visual question answering. We are interested in solving this task in the unsupervised fashion, since obtaining the annotated labels may be a costly affair involving human effort. It has been observed that learning object-centric representations can have a significant advantage, compared to non-object aware approaches, due to their ability to disentangle the scene dyanamics over movement of individual objects. While some of the existing approaches work with a disentangled representation of individual objects~\cite{}, some of the most recent work represents each object as a single dense vector. 

%Inspired by the fact that not all the object attributes are relevant for dynamics prediction, we ask the following questions (a) Is it possible to extract a disentangled object representation in terms of its natural attributes such as color, size, position etc. (b) does such a distentangled representation help better learn visual dynamics. While their has been some work, which has attempted to do so~\cite{}, the results have been far from optimal. Either, they make strong limiting assumptions about the kind of objects present in the image, or do not exploit the learned representattion explicitly for dynamics prediction.

%In this work, we would like to ask the following question: 


%Recent literature has received significant attention for solving the task of unsupervised visual dynamics. Predicting 

%in the task of unsupervised activity recognition. This is an important task by itself, with several applications including in Computer Vision, and Reinforcement Learning. Dealing with the problem in the unsupervised setting is also important, since assuming labeled data is not feasible for every new setting one encounters, and involves a significant labeling cost.  A series of works have been proposed that successively improve the performance of various models on this task~\cite{}.  Often, these approaches have also been referred to as the problem of learning World Models, since the goal is to build a model for the underlying transition for the state change. There is an important representation question here: what is the right latent representation for the underlying image, which is most effective at predicting the future state? While earlier works would assume dense representation for objects, recently, it has been realized that working with object-centric representations has a significant advantage, when it comes to understanding the dynamics and building an effective world model.
%The champions of this line of work include STOVE~\cite{}, GSWM~\cite{}, and SLOTFomer~\cite{}. Interestingly, while all of these approaches make use of a factored representation in terms of decomposing the world into specific objects, it is not entirely clear, if such a representation can be broken down further in terms of object attributes. Presumably, having such a fine-grained representation would not only help disentangle the factors of variation, it also help improve the predictive accuracy.

%While some of the earlier works~\cite{} do have some kind of attribute-based representation for each object, the latter works~\cite{} have disregarded such an explicit 
%representation and only focused on dense object representation in terms of slots ~\cite{}. Presumably, much of their advantage comes from the use of all-powerful transformer-based models. On the other hand, even when dealing with factored representation for each object~\cite{}, earlier work has not explicitly used this in their dynamics prediction module, which we believe is a significant limitation. In this paper, we thought of combining the two lines of work, where inspired by some of the ideas in the earlier works, which make use of disentangled representation for objects, while at the same time, having a transformer-based architecture, resulting in a system which we refer to as {\em DisFormer}.

% \vscom{Next two paragraphs should be rewritten so that process/architecture/approach and contributions get segregated clearly.}

Our work, in the form of DisFormer, presents several novel contributions. %ideas. Our work makes several novel contributions. 
Starting with masks extracted from an object extractor, our key idea is to represent each object as a set of blocks, where each block is expressed as a linear combination of underlying (learned) concepts. Intuitively, each block (or a set of blocks) can be thought of as potentially representing an underlying natural attribute of an object (e.g., size, colour etc.). 
%{\bf Question: Have we looked at what each concept represents? What if we replace an object attribute value with the learned concept value?}. 
While such an idea has been explored in earlier work~\cite{Neural-Systematic-Binder}, it is limited to the case of static images, whereas our goal is to tie the learned representation with dynamics prediction, resulting in some significant technical differences. 
%they only work with static images, whereas our focus is on video prediction, and therefore discovered attributes have to be tied to the underlying dynamics. 
In order to learn the individual block representation, we use the notion of a slot~\cite{SLOT-ATTENTION}. Whereas in the original slot attention paper, each slot binds to a particular object, and its representation is obtained by iteratively refining a vector attending over the entire image, in our case, each slot represents a block, which attends over an object, and its iterative refinement results in the final representation of the block. Disentanglement is guided by forcing each block to be a linear combination of a small number of learned concepts. The final object representation is the concatenation of the blocks. 
%representation.
%its the iteratively refinement results in the disentangled reperesentation for each block.

%taking the attention over the entire image, our slots represent blocks, with attention taken over an object, whose iterative refinement results in a disentangled representation.
%and iterative refinement results in a disentangled block representation.

%where each slot represents its binding to a particular block, and is obtained by iteratively refining the attention vector over the entire object representation. Note that this is contrast with the original slot-attention paper, where each slot binds to an object in the image, and attention is taken over the entire image. The final object representation is the concatenation of the blocks. 

For dynamics prediction, we pass the latent representation for the entire set of extracted objects in the image, along with one for the background, to a transformer. A position embedding for each block distinguishes it from others. Since object masks can be discovered in any order, we need to impose a canonical ordering over them so that loss can be taken for the final image. This is done via a novel permutation module, which learns to map object representations to a canonical ordering starting from any given ordering over them. Finally, instead of passing the object representation as a single vector during decoding, we directly map the discovered blocks to individual channels, further reinforcing the discovery of a disentangled representation.
%fact that each block represents a distinct feature of the object.
%discovery of a disentangled representation.
%at each of them represents a distinct feature in the object representation. 
For the object extractor, we make use of a Mask-RCNN trained on labels provided by an unsupervised extractor~\cite{icswm}, for 2D scenes, and slot attention~\cite{SLOT-ATTENTION}, for the case of 3D scenes. For our decoder, we use a standard architecture~\cite{sbd} along with mapping of attribute representation to channels as described above. 

Extensive experimentation on both 2D and 3D datasets shows that our approach outperforms existing SOTA baselines both in terms of pixel error and dynamics, for up to 15 steps of prediction.
% Further, we show that our learned representations are disentangled, resulting in {\em content aware} \vscom{we decided on using content consistent} predictions, where the errors produced by our model are primarily position errors, compared to other approaches which start distorting object attributes, for longer horizon predictions.
Further, we create transfer datasets for 2D environments and 
% \sout{We show that our model has a respectable performance in zero-shot setting, whereas other models fail miserably.}
we observe that our model performs much better in zero-shot settings than the baselines that fail miserably\footnote{We will release our code and datasets for further research after acceptance.}. The rest of the paper is organized as follows: in section~\ref{sec:related}, we will discuss the related work, and in section~\ref{sec:theory}, we will propose our architecture. Section~\ref{sec:expt} discusses the experiments and results, followed by a conclusion and discussion on future work in section~\ref{sec:conclusion}.
